Multi-modal Point-of-Care Diagnostics for COVID-19 Based On Acoustics and Symptoms

The research direction of identifying acoustic bio-markers of respiratory diseases has received renewed interest following the onset of COVID-19 pandemic. In this paper, we design an approach to COVID-19 diagnostic using crowd-sourced multi-modal data. The data resource, consisting of acoustic signals like cough, breathing, and speech signals, along with the data of symptoms, are recorded using a web-application over a period of ten months. We investigate the use of statistical descriptors of simple time-frequency features for acoustic signals and binary features for the presence of symptoms. Unlike previous works, we primarily focus on the application of simple linear classifiers like logistic regression and support vector machines for acoustic data while decision tree models are employed on the symptoms data. We show that a multi-modal integration of acoustics and symptoms classifiers achieves an area-under-curve (AUC) of 92.40, a significant improvement over any individual modality. Several ablation experiments are also provided which highlight the acoustic and symptom dimensions that are important for the task of COVID-19 diagnostics.

==> literature_review_table.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{Ref} &
  \multirow{2}{*}{Features} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dataset size\\ neg/pos\end{tabular}} &
  \multirow{2}{*}{Classifier} &
  \multicolumn{3}{c}{Performance} \\ \cline{5-7} 
 &
   &
   &
   &
  AUC(\%) &
  Sensitivity(\%) &
  Specificity(\%) \\ \hline
 \rowcolor{Gray}
\cite{agbley2020wavelet} &
  \begin{tabular}[c]{@{}c@{}}Wavelet, \\ clinical information based feats\end{tabular} &
  1116/340 &
  Fusion Based Classification &
  - &
  43 &
  81 \vspace{1mm}\\ %\hline
\cite{mouawad2021robust} &
%Symbolic recurrence quantification\\  measures with 13 dim MFCC features
  \begin{tabular}[c]{@{}c@{}}Symbolic recurrence \\ quantification measures  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}} Coughs:1895/32\\ Vowels:1468/20  \end{tabular} &
  XGBoost classifier &
  \begin{tabular}[c]{@{}c@{}}Coughs: 84 \\ Vowel:86\end{tabular} &
  - &
  -   \vspace{1mm}\\
  %\hline
  \rowcolor{Gray}
\cite{laguarta2020COVID} &
  MFCC &
  2660/2660 &
  3 ResNet50 in parallel &
  97 &
  98.5 &
  94.2 \vspace{2mm}\\ %\hline
\cite{brown2020exploring} &
%file level VGGish
  \begin{tabular}[c]{@{}c@{}}Pool of features,  \\ VGGish embeddings\end{tabular} &
  220/62 &
  LogReg, SVM &
  80 &
  - &
  - \vspace{1mm}\\ %\hline
  \rowcolor{Gray}
\cite{imran2020ai4COVID} &
  MFCC &
  247/70 &
  CNN based classifier &
  89.52 &
  - &
  - \vspace{1mm}\\ %\hline
  
\cite{quatieri2020framework} &
  \begin{tabular}[c]{@{}c@{}}Speech envelope, Pitch, \\ Cepstral peak ,formant\end{tabular} &
  %5 subjects speech taken from social \\ media interviews(before and after COVID)
  \begin{tabular}[c]{@{}c@{}}5 \end{tabular} &
  Cohen's d score &
  - &
  - &
  - \vspace{1mm}\\ %\hline
   \rowcolor{Gray}
  \vspace{1mm}
\cite{al2021detection} &
  \begin{tabular}[c]{@{}c@{}}Model Parameter of vocal fold,\\ Residual Coefficient\end{tabular} &
  10/9 &
  %}Logistic regression, SVM with a nonlinear radial basis \\ function kernel, Decision tree, Random forest, AdaBoost
  \begin{tabular}[c]{@{}c@{}}LR, SVM, Decision Tree, \\Random Forest, Adaboost\end{tabular} &
  91 &
  - &
  - \vspace{1mm} \\ %\hline
  
\cite{coppock2021end} &
  Log Spectrogram &
  355/62 &
  COVID-19 Identification ResNet (CIdeR) &
  84.6 &
  - &
  - \vspace{1mm} \\ \hline
\end{tabular}%
}
\caption{\label{tab:lit_review}A listing of literature on acoustics based COVID-19 diagnosis.}
\end{table*}

==> plots/tables/Functionals_details.tex <==
\begin{sidewaystable*}[t!]
    \centering
    \caption{List of statistical features  derived from low-level descriptors given in Table~\ref{tab:llds} \cite{functionals}.}
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
\multirow{2}{*}{Statistic features derived from LLD}           & No.  & \multicolumn{2}{c|}{Spectral \& Energy} & \multicolumn{2}{c|}{Voicing} &  \multirow{2}{*}{Group}       \\ 
& Func.  & LLD & $\Delta$ LLD & LLD & $\Delta$ LLD &       \\ \hline

Quartiles 1–3, 3 inter-quartile ranges & 6 & \checkmark & \checkmark & \checkmark & \checkmark & \multirow{3}{*}{Percentiles (9)} \\ 
$1\%$ percentile ($\sim$ min), $99\%$ percentile ($\sim$ max) & 2 & \checkmark& \checkmark & \checkmark & \checkmark & \\ 
Percentile range 1 \%–99 \%                      & 1 & \checkmark & \checkmark & \checkmark & \checkmark &\\ \hline
Position of min / max, range (max – min) & 3 & \checkmark & \checkmark & \checkmark & \checkmark & \multirow{7}{*}{Temporal (15)}    \\
Contour centroid              & 1  & \checkmark &  &    \checkmark & \checkmark&\\
Contour flatness              & 1  & \checkmark & \checkmark  & \checkmark & \checkmark &   \\
Rel. duration LLD is $> 25~/~50~/75~/90\%$ range & 4 & \checkmark & \checkmark &\checkmark & \checkmark&    \\
Relative duration LLD is rising                  & 1 & \checkmark & \checkmark & \checkmark & \checkmark&   \\
Relative duration LLD has positive curvature        & 1 & \checkmark & \checkmark  &    \checkmark & \checkmark&\\
Mean, max, min, std. deviation of segment length      & 4 & \checkmark & \checkmark$^*$ &  & &  \\
%Percentage of non-zero frames (Only for F0)     & 1 &  & &  && \\
\hline
Mean value of peaks                             & 1 & \checkmark & \checkmark &&& \multirow{6}{*}{Peaks (12)}       \\ 
Mean value of peaks – arithmetic mean            & 1 & \checkmark & \checkmark &   &&   \\ 
Mean / std.deviation of inter peak distances    & 2   & \checkmark & \checkmark    &  &&     \\ 
Amplitude mean of peaks, of minima              & 2  & \checkmark & \checkmark &    && \\ 
Amplitude range of peaks                         & 2 & \checkmark  & \checkmark &    &&\\ 
Mean / std. deviation of rising / falling slopes    & 4 & \checkmark & \checkmark &  &  &      \\ \hline
Arithmetic mean        & 1 & \checkmark &   &\checkmark & \checkmark  & \multirow{4}{*}{Moments (6)}     \\ 
Root quadratic mean        & 1 & \checkmark & \checkmark  &\checkmark & \checkmark  &      \\ 
Positive arithmetic mean        & 1 &  & \checkmark  &\checkmark & \checkmark  &      \\ 
Standard deviation, skewness, kurtosis        & 3  & \checkmark & \checkmark  &  \checkmark & \checkmark &\\ \hline
Linear regression slope, offset, quadratic error & 3 & \checkmark & &\checkmark & \checkmark& \multirow{2}{*}{Regression (7)}  \\ 
Quadratic regression a, b, offset, quadratic error & 4 & \checkmark &  &\checkmark & \checkmark& \\ \hline
Linear prediction (LP) gain, LP Coefficients 1–5 & 6  & \checkmark & \checkmark &\checkmark & \checkmark & {Modulation (6)}  \\ \hline
%\multicolumn{2}{c|}{\bf Total functionals} & {\bf 54} & {\bf 46} & {\bf 39} & {\bf 39} & \\\hline
\multicolumn{7}{c}{1. For F0 LLD, additionally, the $4$ segment length related LLDs and $1$ percentage of non-zero frames functionals are applied.  }\\
\multicolumn{7}{c}{2. Total number of functionals applied is $100$ for spectral and energy LLDs, $78$ for voicing related LLDs except F0, and $83$ for F0. }\\
    \end{tabular}
    \label{tab:functionalsV2}
\end{sidewaystable*}
